Localized emission in MoSe$_2$ monolayers on GaN nanopillars

Solid-state quantum emitters (QEs) in two-dimensional semiconductors offer compact, chip-compatible sources for quantum photonics. In transition-metal dichalcogenides (TMDs), nanopillars are widely used to induce localized emission, yet the underlying confinement mechanism and the relative roles of strain versus dielectric environment remain unclear. The general problem addressed here is whether strain alone explains quantum emitter formation and placement in MoSe$_2$, or whether dielectric contrast at suspended-supported interfaces is also required. Here, we combine hyperspectral superlocalization of photoluminescence with co-registered AFM topography and phase to map the positions of localized states (LS) in MoSe$_2$ suspended on GaN pillars and correlate them with bending strain and the local dielectric context. Contrary to the common assumption of purely strain-driven activation, LS frequently occur at suspended--supported interfaces around the pillar apex and span a broad strain range without a clear threshold, while being scarce along high-strain ripples. Our data indicate that deterministic emitter positioning in Mo-based TMDs benefits from co-engineering both strain gradients and nanoscale dielectric heterogeneity, rather than strain alone. More broadly, this combined optical-mechanical characterization approach provides a general framework for mapping structure-property relationships in 2D quantum materials at the single-emitter level.

==> refs_thebibliography.tex <==
\begin{thebibliography}{99}
\bibitem{agarwal_situ_2025} Agarwal, Hitesh, Reserbat-Plantey, Antoine, Ruiz, David Barcons, Soundarapandian, Karuppasammy, Li, Geng, Mkhitaryan, Vahagn, Osmond, Johann, Lozano, Helena, Watanabe, Kenji, Taniguchi, Takashi, Stepanov, Petr, Koppens, Frank H. L., Kumar, Roshan Krishna, ``In situ engineering hexagonal boron nitride in van der {Waals} heterostructures with selective {SF6} etching'', arXiv, (2025), doi:10.48550/arXiv.2503.14238.

\bibitem{palacios-berraquero_large-scale_2017} Palacios-Berraquero, Carmen, Kara, Dhiren M., Montblanch, Alejandro R.-P., Barbone, Matteo, Latawiec, Pawel, Yoon, Duhee, Ott, Anna K., Loncar, Marko, Ferrari, Andrea C., Atat{\"u}re, Mete, ``Large-scale quantum-emitter arrays in atomically thin semiconductors'', Nature Communications, \textbf{8}(1), 15093, (2017), doi:10.1038/ncomms15093.

\bibitem{aharonovich_solid-state_2016} Aharonovich, Igor, Englund, Dirk, Toth, Milos, ``Solid-state single-photon emitters'', Nature Photonics, \textbf{10}(10), 631--641, (2016), doi:10.1038/nphoton.2016.186.

\bibitem{azzam_prospects_2021} Azzam, Shaimaa I., Parto, Kamyar, Moody, Galan, ``Prospects and challenges of quantum emitters in {2D} materials'', Applied Physics Letters, \textbf{118}(24), 240502, (2021), doi:10.1063/5.0054116.

\bibitem{zhao_single_2018} Zhao, Shen, Lavie, Julien, Rondin, Lo{\"i}c, Orcin-Chaix, Lucile, Diederichs, Carole, Roussignol, Philippe, Chassagneux, Yannick, Voisin, Christophe, M{\"u}llen, Klaus, Narita, Akimitsu, Campidelli, St{\'e}phane, Lauret, Jean-S{\'e}bastien, ``Single photon emission from graphene quantum dots at room temperature'', Nature Communications, \textbf{9}(1), 3470, (2018), doi:10.1038/s41467-018-05888-w.

\bibitem{toninelli_single_2021} Toninelli, C., Gerhardt, I., Clark, A. S., Reserbat-Plantey, A., G{\"o}tzinger, S., Ristanovi{\'c}, Z., Colautti, M., Lombardi, P., Major, K. D., Deperasi{\'n}ska, I., Pernice, W. H., Koppens, F. H. L., Kozankiewicz, B., Gourdon, A., Sandoghdar, V., Orrit, M., ``Single organic molecules for photonic quantum technologies'', Nature Materials, \textbf{20}(12), 1615--1628, (2021), doi:10.1038/s41563-021-00987-4.

\bibitem{he_carbon_2018} He, X., Htoon, H., Doorn, S. K., Pernice, W. H. P., Pyatkov, F., Krupke, R., Jeantet, A., Chassagneux, Y., Voisin, C., ``Carbon nanotubes as emerging quantum-light sources'', Nature Materials, \textbf{17}(8), 663--670, (2018), doi:10.1038/s41563-018-0109-2.

\bibitem{tonndorf_single-photon_2015} Tonndorf, Philipp, Schmidt, Robert, Schneider, Robert, Kern, Johannes, Buscema, Michele, Steele, Gary A., Castellanos-Gomez, Andres, Zant, Herre S. J. van der, Vasconcellos, Steffen Michaelis de, Bratschitsch, Rudolf, ``Single-photon emission from localized excitons in an atomically thin semiconductor'', Optica, \textbf{2}(4), 347--352, (2015), doi:10.1364/OPTICA.2.000347.

\bibitem{srivastava_optically_2015} Srivastava, Ajit, Sidler, Meinrad, Allain, Adrien V., Lembke, Dominik S., Kis, Andras, Imamo{\char287}lu, A., ``Optically active quantum dots in monolayer {WSe2}'', Nature Nanotechnology, \textbf{10}(6), 491--496, (2015), doi:10.1038/nnano.2015.60.

\bibitem{koperski_single_2015} Koperski, M., Nogajewski, K., Arora, A., Cherkez, V., Mallet, P., Veuillen, J.-Y., Marcus, J., Kossacki, P., Potemski, M., ``Single photon emitters in exfoliated {WSe2} structures'', Nature Nanotechnology, \textbf{10}(6), 503--506, (2015), doi:10.1038/nnano.2015.67.

\bibitem{he_single_2015} He, Yu-Ming, Clark, Genevieve, Schaibley, John R., He, Yu, Chen, Ming-Cheng, Wei, Yu-Jia, Ding, Xing, Zhang, Qiang, Yao, Wang, Xu, Xiaodong, Lu, Chao-Yang, Pan, Jian-Wei, ``Single quantum emitters in monolayer semiconductors'', Nature Nanotechnology, \textbf{10}(6), 497--502, (2015), doi:10.1038/nnano.2015.75.

\bibitem{rosenberger_quantum_2019} Rosenberger, Matthew R., Dass, Chandriker Kavir, Chuang, Hsun-Jen, Sivaram, Saujan V., McCreary, Kathleen M., Hendrickson, Joshua R., Jonker, Berend T., ``Quantum {Calligraphy}: {Writing} {Single}-{Photon} {Emitters} in a {Two}-{Dimensional} {Materials} {Platform}'', ACS Nano, \textbf{13}(1), 904--912, (2019), doi:10.1021/acsnano.8b08730.

\bibitem{chakraborty_voltage-controlled_2015} Chakraborty, Chitraleema, Kinnischtzke, Laura, Goodfellow, Kenneth M., Beams, Ryan, Vamivakas, A. Nick, ``Voltage-controlled quantum light from an atomically thin semiconductor'', Nature Nanotechnology, \textbf{10}(6), 507--511, (2015), doi:10.1038/nnano.2015.79.

\bibitem{heithoff_valley-hybridized_2024} Heithoff, Maximilian, Moreno, {\'A}lvaro, Torre, Iacopo, Feuer, Matthew S. G., Purser, Carola M., Andolina, Gian Marcello, Calaj{\`o}, Giuseppe, Watanabe, Kenji, Taniguchi, Takashi, Kara, Dhiren M., Hays, Patrick, Tongay, Seth Ariel, Fal'ko, Vladimir I., Chang, Darrick, Atat{\"u}re, Mete, Reserbat-Plantey, Antoine, Koppens, Frank H.L., ``Valley-{Hybridized} {Gate}-{Tunable} {1D} {Exciton} {Confinement} in {MoSe2}'', ACS Nano, \textbf{18}(44), 30283--30292, (2024), doi:10.1021/acsnano.4c04786.

\bibitem{thureja_electrically_2022} Thureja, Deepankur, Imamoglu, Atac, Smole{\'n}ski, Tomasz, Amelio, Ivan, Popert, Alexander, Chervy, Thibault, Lu, Xiaobo, Liu, Song, Barmak, Katayun, Watanabe, Kenji, Taniguchi, Takashi, Norris, David J., Kroner, Martin, Murthy, Puneet A., ``Electrically tunable quantum confinement of neutral excitons'', Nature, \textbf{606}(7913), 298--304, (2022), doi:10.1038/s41586-022-04634-z.

\bibitem{thureja_electrically_2024} Thureja, Deepankur, Yaz{\char305}c{\char305}, F. Emre, Smole{\'n}ski, Tomasz, Kroner, Martin, Norris, David J., {\char304}mamo{\char487}lu, Atac, ``Electrically defined quantum dots for bosonic excitons'', Physical Review B, \textbf{110}(24), 245425, (2024), doi:10.1103/PhysRevB.110.245425.

\bibitem{baek_highly_2020} Baek, H., Brotons-Gisbert, M., Koong, Z. X., Campbell, A., Rambach, M., Watanabe, K., Taniguchi, T., Gerardot, B. D., ``Highly energy-tunable quantum light from moir{\'e}-trapped excitons'', Science Advances, \textbf{6}(37), eaba8526, (2020), doi:10.1126/sciadv.aba8526.

\bibitem{seyler_signatures_2019} Seyler, Kyle L., Rivera, Pasqual, Yu, Hongyi, Wilson, Nathan P., Ray, Essance L., Mandrus, David G., Yan, Jiaqiang, Yao, Wang, Xu, Xiaodong, ``Signatures of moir{\'e}-trapped valley excitons in {MoSe2}/{WSe2} heterobilayers'', Nature, \textbf{567}(7746), 66--70, (2019), doi:10.1038/s41586-019-0957-1.

\bibitem{branny_deterministic_2017} Branny, Artur, Kumar, Santosh, Proux, Rapha{\"e}l, Gerardot, Brian D., ``Deterministic strain-induced arrays of quantum emitters in a two-dimensional semiconductor'', Nature Communications, \textbf{8}(1), 15053, (2017), doi:10.1038/ncomms15053.

\bibitem{kim_position_2019} Kim, Hyoju, Moon, Jong Sung, Noh, Gichang, Lee, Jieun, Kim, Je-Hyung, ``Position and {Frequency} {Control} of {Strain}-{Induced} {Quantum} {Emitters} in {WSe}$_{\textrm{2}}$ {Monolayers}'', Nano Letters, \textbf{19}(10), 7534--7539, (2019), doi:10.1021/acs.nanolett.9b03421.

\bibitem{luo_deterministic_2018} Luo, Yue, Shepard, Gabriella D., Ardelean, Jenny V., Rhodes, Daniel A., Kim, Bumho, Barmak, Katayun, Hone, James C., Strauf, Stefan, ``Deterministic coupling of site-controlled quantum emitters in monolayer {WSe}$_{\textrm{2}}$ to plasmonic nanocavities'', Nature Nanotechnology, \textbf{13}(12), 1137--1142, (2018), doi:10.1038/s41565-018-0275-z.

\bibitem{linhart_localized_2019} Linhart, Lukas, Paur, Matthias, Smejkal, Valerie, Burgd{\"o}rfer, Joachim, Mueller, Thomas, Libisch, Florian, ``Localized {Intervalley} {Defect} {Excitons} as {Single}-{Photon} {Emitters} in \$\{{\textbackslash}mathrm\{{WSe}\}\}\_\{2\}\$'', Physical Review Letters, \textbf{123}(14), 146401, (2019), doi:10.1103/PhysRevLett.123.146401.

\bibitem{kern_nanoscale_2016} Kern, Johannes, Niehues, Iris, Tonndorf, Philipp, Schmidt, Robert, Wigger, Daniel, Schneider, Robert, Stiehm, Torsten, Michaelis de Vasconcellos, Steffen, Reiter, Doris E., Kuhn, Tilmann, Bratschitsch, Rudolf, ``Nanoscale {Positioning} of {Single}-{Photon} {Emitters} in {Atomically} {Thin} {WSe2}'', Advanced Materials, \textbf{28}(33), 7101--7105, (2016), doi:10.1002/adma.201600560.

\bibitem{fournier_position-controlled_2021} Fournier, Clarisse, Plaud, Alexandre, Roux, S{\'e}bastien, Pierret, Aur{\'e}lie, Rosticher, Michael, Watanabe, Kenji, Taniguchi, Takashi, Buil, St{\'e}phanie, Qu{\'e}lin, Xavier, Barjon, Julien, Hermier, Jean-Pierre, Delteil, Aymeric, ``Position-controlled quantum emitters with reproducible emission wavelength in hexagonal boron nitride'', Nature Communications, \textbf{12}(1), 3779, (2021), doi:10.1038/s41467-021-24019-6.

\bibitem{parto_defect_2021} Parto, Kamyar, Azzam, Shaimaa I., Banerjee, Kaustav, Moody, Galan, ``Defect and strain engineering of monolayer {WSe2} enables site-controlled single-photon emission up to 150 {K}'', Nature Communications, \textbf{12}(1), 3585, (2021), doi:10.1038/s41467-021-23709-5.

\bibitem{klein_site-selectively_2019} Klein, J., Lorke, M., Florian, M., Sigger, F., Sigl, L., Rey, S., Wierzbowski, J., Cerne, J., M{\"u}ller, K., Mitterreiter, E., Zimmermann, P., Taniguchi, T., Watanabe, K., Wurstbauer, U., Kaniber, M., Knap, M., Schmidt, R., Finley, J. J., Holleitner, A. W., ``Site-selectively generated photon emitters in monolayer {MoS2} via local helium ion irradiation'', Nature Communications, \textbf{10}(1), 2755, (2019), doi:10.1038/s41467-019-10632-z.

\bibitem{asenjo-garcia_exponential_2017} Asenjo-Garcia, A., Moreno-Cardoner, M., Albrecht, A., Kimble, H.{\char8201}J., Chang, D.{\char8201}E., ``Exponential {Improvement} in {Photon} {Storage} {Fidelities} {Using} {Subradiance} and "{Selective} {Radiance}" in {Atomic} {Arrays}'', Physical Review X, \textbf{7}(3), 031024, (2017), doi:10.1103/PhysRevX.7.031024.

\bibitem{wang_utilizing_2022} Wang, Wei, Jones, Leighton O., Chen, Jia-Shiang, Schatz, George C., Ma, Xuedan, ``Utilizing {Ultraviolet} {Photons} to {Generate} {Single}-{Photon} {Emitters} in {Semiconductor} {Monolayers}'', ACS Nano, \textbf{16}(12), 21240--21247, (2022), doi:10.1021/acsnano.2c09209.

\bibitem{raja_coulomb_2017} Raja, Archana, Chaves, Andrey, Yu, Jaeeun, Arefe, Ghidewon, Hill, Heather M., Rigosi, Albert F., Berkelbach, Timothy C., Nagler, Philipp, Sch{\"u}ller, Christian, Korn, Tobias, Nuckolls, Colin, Hone, James, Brus, Louis E., Heinz, Tony F., Reichman, David R., Chernikov, Alexey, ``Coulomb engineering of the bandgap and excitons in two-dimensional materials'', Nature Communications, \textbf{8}(1), 15251, (2017), doi:10.1038/ncomms15251.

\bibitem{ben_mhenni_breakdown_2025} Ben Mhenni, Amine, Van Tuan, Dinh, Geilen, Leonard, Petri{\'c}, Marko M., Erdi, Melike, Watanabe, Kenji, Taniguchi, Takashi, Tongay, Seth Ariel, M{\"u}ller, Kai, Wilson, Nathan P., Finley, Jonathan J., Dery, Hanan, Barbone, Matteo, ``Breakdown of the {Static} {Dielectric} {Screening} {Approximation} of {Coulomb} {Interactions} in {Atomically} {Thin} {Semiconductors}'', ACS Nano, \textbf{19}(4), 4269--4278, (2025), doi:10.1021/acsnano.4c11563.

\bibitem{itzhak_exciton_2025} Itzhak, Raziel, Suleymanov, Nathan, Minkovich, Boris, Kartvelishvili, Liana, Kostianovski, Vladislav, Korobko, Roman, Hayat, Alex, Goykhman, Ilya, ``Exciton {Manipulation} via {Dielectric} {Environment} {Engineering} in {2D} {Semiconductors}'', ACS Applied Optical Materials, \textbf{3}(6), 1330--1338, (2025), doi:10.1021/acsaom.5c00105.

\bibitem{noauthor_coupling_nodate} ``Coupling {Single} {Photons} from {Discrete} {Quantum} {Emitters} in {WSe2} to {Lithographically} {Defined} {Plasmonic} {Slot} {Waveguides} {\textbar} {Nano} {Letters}''.

\bibitem{blauth_coupling_2018} Blauth, M., J{\"u}rgensen, M., Vest, G., Hartwig, O., Prechtl, M., Cerne, J., Finley, J. J., Kaniber, M., ``Coupling {Single} {Photons} from {Discrete} {Quantum} {Emitters} in {WSe2} to {Lithographically} {Defined} {Plasmonic} {Slot} {Waveguides}'', Nano Letters, \textbf{18}(11), 6812--6819, (2018), doi:10.1021/acs.nanolett.8b02687.

\bibitem{xu_subdiffraction_2024} Xu, David D., Vong, Albert F., Utama, M. Iqbal Bakti, Lebedev, Dmitry, Ananth, Riddhi, Hersam, Mark C., Weiss, Emily A., Mirkin, Chad A., ``Sub{\char8208}{Diffraction} {Correlation} of {Quantum} {Emitters} and {Local} {Strain} {Fields} in {Strain}{\char8208}{Engineered} {WSe} 2 {Monolayers}'', Advanced Materials, \textbf{36}(25), (2024), doi:10.1002/adma.202314242.

\bibitem{abramov_photoluminescence_2023} Abramov, Artem N., Chestnov, Igor Y., Alimova, Ekaterina S., Ivanova, Tatiana, Mukhin, Ivan S., Krizhanovskii, Dmitry N., Shelykh, Ivan A., Iorsh, Ivan V., Kravtsov, Vasily, ``Photoluminescence imaging of single photon emitters within nanoscale strain profiles in monolayer {WSe2}'', Nature Communications, \textbf{14}(1), 5737, (2023), doi:10.1038/s41467-023-41292-9.

\bibitem{luo_imaging_2023} Luo, Weijun, Lawrie, Benjamin J., Puretzky, Alexander A., Tan, Qishuo, Gao, Hongze, Lingerfelt, David B., Eichman, Gage, Mcgee, Edward, Swan, Anna K., Liang, Liangbo, Ling, Xi, ``Imaging {Strain}-{Localized} {Single}-{Photon} {Emitters} in {Layered} {GaSe} below the {Diffraction} {Limit}'', ACS Nano, \textbf{17}(23), 23455--23465, (2023), doi:10.1021/acsnano.3c05250.

\bibitem{yu_site-controlled_2021} Yu, Leo, Deng, Minda, Zhang, Jingyuan Linda, Borghardt, Sven, Kardynal, Beata, Vu{\char269}kovi{\'c}, Jelena, Heinz, Tony F., ``Site-{Controlled} {Quantum} {Emitters} in {Monolayer} {MoSe2}'', Nano Letters, \textbf{21}(6), 2376--2381, (2021), doi:10.1021/acs.nanolett.0c04282.

\bibitem{kim_confinement_2024} Kim, Gwangwoo, Huet, Benjamin, Stevens, Christopher E., Jo, Kiyoung, Tsai, Jeng-Yuan, Bachu, Saiphaneendra, Leger, Meghan, Song, Seunguk, Rahaman, Mahfujur, Ma, Kyung Yeol, Glavin, Nicholas R., Shin, Hyeon Suk, Alem, Nasim, Yan, Qimin, Hendrickson, Joshua R., Redwing, Joan M., Jariwala, Deep, ``Confinement of excited states in two-dimensional, in-plane, quantum heterostructures'', Nature Communications, \textbf{15}(1), 6361, (2024), doi:10.1038/s41467-024-50653-x.

\bibitem{akinwande_graphene_2019} Akinwande, Deji, Huyghebaert, Cedric, Wang, Ching-Hua, Serna, Martha I., Goossens, Stijn, Li, Lain-Jong, Wong, H.-S. Philip, Koppens, Frank H. L., ``Graphene and two-dimensional materials for silicon technology'', Nature, \textbf{573}(7775), 507--518, (2019), doi:10.1038/s41586-019-1573-9.

\bibitem{hu_quantum_2024} Hu, Jenny, Lorchat, Etienne, Chen, Xueqi, Watanabe, Kenji, Taniguchi, Takashi, Heinz, Tony F., Murthy, Puneet A., Chervy, Thibault, ``Quantum control of exciton wave functions in {2D} semiconductors'', Science Advances, \textbf{10}(12), eadk6369, (2024), doi:10.1126/sciadv.adk6369.

\bibitem{barcons_ruiz_engineering_2022} Barcons Ruiz, David, Herzig Sheinfux, Hanan, Hoffmann, Rebecca, Torre, Iacopo, Agarwal, Hitesh, Kumar, Roshan Krishna, Vistoli, Lorenzo, Taniguchi, Takashi, Watanabe, Kenji, Bachtold, Adrian, Koppens, Frank H. L., ``Engineering high quality graphene superlattices via ion milled ultra-thin etching masks'', Nature Communications, \textbf{13}(1), 6926, (2022), doi:10.1038/s41467-022-34734-3.

\bibitem{soubelet_strong_2025} Soubelet, Pedro, Tong, Yao, Astaburuaga Hernandez, Asier, Ji, Peirui, Gallo, Katia, Stier, Andreas V., Finley, Jonathan J., ``Strong {Quantum} {Confinement} of {2D} {Excitons} in an {Engineered} {1D} {Potential} {Induced} by {Proximal} {Ferroelectric} {Domain} {Walls}'', Nano Letters, \textbf{25}(34), 12842--12850, (2025), doi:10.1021/acs.nanolett.5c02438.

\bibitem{hernandez_lopez_strain_2022} Hern{\'a}ndez L{\'o}pez, Pablo, Heeg, Sebastian, Schattauer, Christoph, Kovalchuk, Sviatoslav, Kumar, Abhijeet, Bock, Douglas J., Kirchhof, Jan N., H{\"o}fer, Bianca, Greben, Kyrylo, Yagodkin, Denis, Linhart, Lukas, Libisch, Florian, Bolotin, Kirill I., ``Strain control of hybridization between dark and localized excitons in a {2D} semiconductor'', Nature Communications, \textbf{13}(1), 7691, (2022), doi:10.1038/s41467-022-35352-9.

\bibitem{raynaud_superlocalization_2019} Raynaud, C., Claude, T., Borel, A., Amara, M. R., Graf, A., Zaumseil, J., Lauret, J.-S., Chassagneux, Y., Voisin, C., ``Superlocalization of {Excitons} in {Carbon} {Nanotubes} at {Cryogenic} {Temperature}'', Nano Letters, \textbf{19}(10), 7210--7216, (2019), doi:10.1021/acs.nanolett.9b02816.

\bibitem{Dirnberger2021} Dirnberger, Florian, Ziegler, Jonas D., Faria Junior, Paulo E., Bushati, Rezlind, Taniguchi, Takashi, Watanabe, Kenji, Fabian, Jaroslav, Bougeard, Dominique, Chernikov, Alexey, Menon, Vinod M., ``Quasi-{1D} exciton channels in strain-engineered {2D} materials'', Science Advances, \textbf{7}(44), (2021), doi:10.1126/sciadv.abj3066.

\bibitem{vasic_phase_2017} Vasi{\'c}, Borislav, Matkovi{\'c}, Aleksandar, Gaji{\'c}, Rado{\char353}, ``Phase imaging and nanoscale energy dissipation of supported graphene using amplitude modulation atomic force microscopy'', Nanotechnology, \textbf{28}(46), 465708, (2017), doi:10.1088/1361-6528/aa8e3b.

\bibitem{semond_gan_1999} Semond, F., Damilano, B., V{\'e}zian, S., Grandjean, N., Leroux, M., Massies, J., ``{GaN} grown on {Si}(111) substrate: {From} two-dimensional growth to quantum well assessment'', Applied Physics Letters, \textbf{75}(1), 82--84, (1999), doi:10.1063/1.124283.

\bibitem{noauthor_properties_nodate} ``Properties of {Advanced} {Semiconductor} {Materials}: {GaN}, {AIN}, {InN}, {BN}, {SiC}, {SiGe} {\textbar} {Wiley}'', Wiley.com.

\bibitem{levinstejn_properties_2001} Levin{\char353}tejn, Michail E., Rumyantsev, Sergey L., Shur, Michael, ``Properties of advanced semiconductor materials {GaN}, {AlN}, {InN}, {BN}, {SiC}, {SiGe}'', Wiley, (2001).

\bibitem{chernikov_exciton_2014} Chernikov, Alexey, Berkelbach, Timothy C., Hill, Heather M., Rigosi, Albert, Li, Yilei, Aslan, Burak, Reichman, David R., Hybertsen, Mark S., Heinz, Tony F., ``Exciton {Binding} {Energy} and {Nonhydrogenic} {Rydberg} {Series} in {Monolayer} \$\{{\textbackslash}mathrm\{{WS}\}\}\_\{2\}\$'', Physical Review Letters, \textbf{113}(7), 076802, (2014), doi:10.1103/PhysRevLett.113.076802.

\bibitem{xu_creation_2021} Xu, Yang, Horn, Connor, Zhu, Jiacheng, Tang, Yanhao, Ma, Liguo, Li, Lizhong, Liu, Song, Watanabe, Kenji, Taniguchi, Takashi, Hone, James C., Shan, Jie, Mak, Kin Fai, ``Creation of moir{\'e} bands in a monolayer semiconductor by spatially periodic dielectric screening'', Nature Materials, \textbf{20}(5), 645--649, (2021), doi:10.1038/s41563-020-00888-y.

\bibitem{van_tuan_effects_2024} Van Tuan, Dinh, Dery, Hanan, ``Effects of dynamical dielectric screening on the excitonic spectrum of monolayer semiconductors'', Physical Review B, \textbf{110}(12), 125301, (2024), doi:10.1103/PhysRevB.110.125301.

\bibitem{daveau_spectral_2020} Daveau, Rapha{\"e}l S., Vandekerckhove, Tom, Mukherjee, Arunabh, Wang, Zefang, Shan, Jie, Mak, Kin Fai, Vamivakas, A. Nick, Fuchs, Gregory D., ``Spectral and spatial isolation of single tungsten diselenide quantum emitters using hexagonal boron nitride wrinkles'', APL Photonics, \textbf{5}(9), 096105, (2020), doi:10.1063/5.0013825.

\bibitem{gelly_probing_2022} Gelly, Ryan J., Renaud, Dylan, Liao, Xing, Pingault, Benjamin, Bogdanovic, Stefan, Scuri, Giovanni, Watanabe, Kenji, Taniguchi, Takashi, Urbaszek, Bernhard, Park, Hongkun, Lon{\char269}ar, Marko, ``Probing dark exciton navigation through a local strain landscape in a {WSe2} monolayer'', Nature Communications, \textbf{13}(1), 232, (2022), doi:10.1038/s41467-021-27877-2.

\bibitem{tripathi_spontaneous_2018} Tripathi, Laxmi Narayan, Iff, Oliver, Betzold, Simon, Dusanowski, {\char321}ukasz, Emmerling, Monika, Moon, Kihwan, Lee, Young Jin, Kwon, Soon-Hong, H{\"o}fling, Sven, Schneider, Christian, ``Spontaneous {Emission} {Enhancement} in {Strain}-{Induced} {WSe2} {Monolayer}-{Based} {Quantum} {Light} {Sources} on {Metallic} {Surfaces}'', ACS Photonics, \textbf{5}(5), 1919--1926, (2018), doi:10.1021/acsphotonics.7b01053.

\bibitem{campo_optical_2021} Campo, Jochen, Cambr{\'e}, Sofie, Botka, Bea, Obrzut, Jan, Wenseleers, Wim, Fagan, Jeffrey A., ``Optical {Property} {Tuning} of {Single}-{Wall} {Carbon} {Nanotubes} by {Endohedral} {Encapsulation} of a {Wide} {Variety} of {Dielectric} {Molecules}'', ACS Nano, \textbf{15}(2), 2301--2317, (2021), doi:10.1021/acsnano.0c08352.

\bibitem{walsh_scaling_2008} Walsh, Andrew G., Nickolas Vamivakas, A., Yin, Yan, Cronin, Stephen B., Selim {\"U}nl{\"u}, M., Goldberg, Bennett B., Swan, Anna K., ``Scaling of exciton binding energy with external dielectric function in carbon nanotubes'', Physica E: Low-dimensional Systems and Nanostructures, \textbf{40}(7), 2375--2379, (2008), doi:10.1016/j.physe.2007.07.007.

\bibitem{ando_environment_2010} Ando, Tsuneya, ``Environment {Effects} on {Excitons} in {Semiconducting} {Carbon} {Nanotubes}'', Journal of the Physical Society of Japan, \textbf{79}(2), 024706, (2010), doi:10.1143/JPSJ.79.024706.

\bibitem{le_louarn_aln_2009} Le Louarn, A., V{\'e}zian, S., Semond, F., Massies, J., ``{AlN} buffer layer growth for {GaN} epitaxy on (1 1 1) {Si}: {Al} or {N} first?'', Journal of Crystal Growth, \textbf{311}(12), 3278--3284, (2009), doi:10.1016/j.jcrysgro.2009.04.001.

\bibitem{park_effect_2014} Park, Young-Shin, Bae, Wan Ki, Padilha, Lazaro A., Pietryga, Jeffrey M., Klimov, Victor I., ``Effect of the {Core}/{Shell} {Interface} on {Auger} {Recombination} {Evaluated} by {Single}-{Quantum}-{Dot} {Spectroscopy}'', Nano Letters, \textbf{14}(2), 396--402, (2014), doi:10.1021/nl403289w.

\bibitem{schermelleh_super-resolution_2019} Schermelleh, Lothar, Ferrand, Alexia, Huser, Thomas, Eggeling, Christian, Sauer, Markus, Biehlmaier, Oliver, Drummen, Gregor P. C., ``Super-resolution microscopy demystified'', Nature Cell Biology, \textbf{21}(1), 72--84, (2019), doi:10.1038/s41556-018-0251-8.

\bibitem{iff_substrate_2017} Iff, Oliver, He, Yu-Ming, Lundt, Nils, Stoll, Sebastian, Baumann, Vasilij, H{\"o}fling, Sven, Schneider, Christian, ``Substrate engineering for high-quality emission of free and localized excitons from atomic monolayers in hybrid architectures'', Optica, \textbf{4}(6), 669--673, (2017), doi:10.1364/OPTICA.4.000669.
\end{thebibliography}

